Minimum Coverage by Convex Polygons: The CG:SHOP Challenge 2023

We give an overview of the 2023 Computational Geometry Challenge targeting the problem Minimum Coverage by Convex Polygons, which consists of covering a given polygonal region (possibly with holes) by a minimum number of convex subsets, a problem with a long-standing tradition in Computational Geometry.

==> Makefile <==
# This is the magic latex makefile composed by Dominik Krupke (krupke@ibr.cs.tu-bs.de) for writing papers.
# You can find the corresponding repository at https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex
# A lot of the ideas are taken and composed from various sources. So feel free to steal it yourself.
-include Makefile.local

# The following variable usually don't need to be altered
TEXFILES:=$(sort $(wildcard *.tex) $(wildcard **/*.tex))

pdf: figures $(TEXFILES)
	latexmk --output-directory=.auxiliary-latex -pdf $(MAIN).tex
	cp ./.auxiliary-latex/$(MAIN).pdf ./$(MAIN).pdf

.DEFAULT_GOAL = all
.PHONY: all check clean

all: pdf

setup: python3
	python3 ./makefile_utils.py --setup

update:
	$(if $(shell command -v wget 2> /dev/null),,$(error Please install `wget` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install wget`))
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/Makefile -O Makefile
	wget https://gitlab.ibr.cs.tu-bs.de/krupke/magic-latex/raw/master/makefile_utils.py -O makefile_utils.py

python3:
	$(if $(shell command -v python3 2> /dev/null),,$(error Please install `python3` to continue. This should be possible with nearly all package managers. On OS X with Homebrew for example via `brew install python`))

figures: python3
	python3 ./makefile_utils.py --svg
	python3 ./makefile_utils.py --ipe

autofix: python3
	python3 ./makefile_utils.py --autofix

check: packagecheck spellcheck grammarcheck phrasingcheck fontcheck texcheck

phrasingcheck: python3
	python3 ./makefile_utils.py --diction

packagecheck: python3
	python3 ./makefile_utils.py --packages

fontcheck: python3
	python3 ./makefile_utils.py --fonts

spellcheck:
	python3 ./makefile_utils.py --spell

grammarcheck: python3
	python3 ./makefile_utils.py --grammar

texcheck:
	python3 ./makefile_utils.py --texlint

reference:
	python3 ./makefile_utils.py --saverevision

clean:
	rm -f $(MAIN).pdf
	rm -rf .auxiliary-latex

showchanges:
ifeq ($(VCS),git)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) --no-pager diff --color-words $$texfile;\
		done
endif
ifeq ($(VCS),svn)
	for texfile in $(TEXFILES); do \
		echo $$texfile; \
		$(VCS) diff $$texfile; \
		done
endif

diff-pdf:
	latexdiff-vc --$(VCS) --flatten -r $(REFERENCE_REVISION) $(MAIN).tex
	latexmk --output-directory=.auxiliary-latex-diff -pdf $(MAIN)-diff$(REFERENCE_REVISION).tex
	cp ./.auxiliary-latex-diff/$(MAIN)-diff$(REFERENCE_REVISION).pdf .
	rm $(MAIN)-diff$(REFERENCE_REVISION).tex


